Winter Wheat Crop Yield Prediction on Multiple Heterogeneous Datasets using Machine Learning

Winter wheat is one of the most important crops in the United Kingdom, and crop yield prediction is essential for the nation's food security. Several studies have employed machine learning (ML) techniques to predict crop yield on a county or farm-based level. The main objective of this study is to predict winter wheat crop yield using ML models on multiple heterogeneous datasets, i.e., soil and weather on a zone-based level. Experimental results demonstrated their impact when used alone and in combination. In addition, we employ numerous ML algorithms to emphasize the significance of data quality in any machine-learning strategy.

==> acronym.tex <==
\newacronym{ai}{AI}{Artificial Intelligence}
\newacronym{cc}{CC}{Cloud Computing}


\newacronym{ml}{ML}{Machine Learning}
\newacronym{et}{ET}{Extra Trees regressor}
\newacronym{rf}{RF}{Random Forest}
\newacronym{cbt}{CBT}{CatBoost regressor}
\newacronym{knn}{KNN}{K nearest neighbour regressor}
\newacronym{dt}{DT}{Decision Tree regressor}
\newacronym{lgbm}{LGBM}{Light Gradient Boosting Machine}
\newacronym{gbt}{GBT}{Gradient Boosting Tree}
\newacronym{xgboost}{XGBoost}{Extreme Gradient Boosting}
\newacronym{lr}{LR}{Linear Regression}
\newacronym{svm}{SVM}{Support Vector Machine}
\newacronym{lasso}{Lasso}{Least absolute shrinkage and selection operator}
\newacronym{ridge}{Ridge}{Ridge regression}
\newacronym{m5}{M5}{M5 Prime Regression}

\newacronym{dl}{DL}{Deep Learning}
\newacronym{nn}{NN}{Neural Networks}
\newacronym{ann}{ANN}{Artificial Neural Networks}
\newacronym{cnn}{CNN}{Convolution Neural Networks}
\newacronym{dnn}{DNN}{Deep Neural Networks}
\newacronym{lstm}{LSTM}{Long short-term memory}
\newacronym{rnn}{RNN}{Recurrent Neural Networks}
\newacronym{bpnn}{BPNN}{Back Propagation Neural Networks}
\newacronym{dtl}{DTL}{Deep Transfer Learning}
\newacronym{mtl}{MTL}{Multi Task Learning}


\newacronym{rs}{RS}{Remote Sensing}
\newacronym{modis}{MODIS}{Moderate Resolution Imaging  Spectro radiometer}
\newacronym{avhrr}{AVHRR}{Advanced  Very  High  Resolution  Radiometer}
\newacronym{ndvi}{NDVI}{Normalized difference vegetation index}
\newacronym{ndwi}{NDVI}{Normalized difference water index}
\newacronym{evi}{EVI}{Enhanced vegetation index}
\newacronym{lai}{LAI}{Leaf Area Index}
\newacronym{fpar}{FPAR}{Fraction of Photo synthetically Active Radiation}
\newacronym{gpp}{GPP}{Gross Primary Production}
\newacronym{uav}{UAV}{Unmanned Aerial Vehicle}
\newacronym{rgb}{RGB}{Red Green Blue}
\newacronym{sif}{SIF}{Sun-induced fluorescence}

\newacronym{gdf}{GDF}{Grouped Data Features}
\newacronym{rmse}{RMSE}{Root Mean Squared Error}

\newacronym{mae}{MAE}{Mean Absolute Error}

